On the $K(1)$-local homotopy of $\mathrm{tmf} \wedge \mathrm{tmf}$

As a step towards understanding the $\mathrm{tmf}$-based Adams spectral sequence, we compute the $K(1)$-local homotopy of $\mathrm{tmf} \wedge \mathrm{tmf}$, using a small presentation of $L_{K(1)}\mathrm{tmf}$ due to Hopkins. We also describe the $K(1)$-local $\mathrm{tmf}$-based Adams spectral sequence.

==> ASS.tex <==
	
\section{Complete Hopf algebroids and Adams spectral sequence}

This section builds on the ideas introduced in \ref{subsec: completeness}, proving additional results useful for work in the $K(1)$-local category. We begin by introducing the important technical notion here is pro-freeness, which appears to be the appropriate replacement for flatness in the $L$-complete setting. As we have to deal with some relative tensor products of $K(1)$-local ring spectra, we need a relative definition of pro-freeness that is more general than that used by other authors, e.~g.~\cite{HoveySS}. We prove some useful algebraic lemmas about this notion, as well as a K\"unneth formula for relative tensor products in which one of the modules is pro-free. This is mostly an easy consequence of work of Hovey and Strickland, and is specific to height 1. We then introduce Baker's concept of $L$-complete Hopf algebroids, and generalize work of Barthel and Heard to show that the $K(1)$-local Adams spectral sequence based on a ring spectrum with an $L$-complete Hopf algebroid is describable in terms of Ext, in certain nice cases.
	
	\begin{defn}
	Let $R_* \in \CAlg_*^\wedge$, and let $M_* \in \Mod_{R_*}^\wedge$. Say that $M_*$ is \textbf{pro-free} if it is of the form
	\[	M_* \cong L_0F_*,	\]
	where $F_*$ is a free graded $R_*$-module. Say that a map $R_* \to S_*$ of commutative rings in $\Mod_*^\wedge$ is \textbf{pro-free} if $S_*$ is a pro-free $R_*$-module.
	\end{defn}
	
	Pro-free modules are projective in the category $\Mod_{R_*}^\wedge$. In this height 1 case, they are also flat. As is shown below, this follows from the fact that direct sums in $\Mod_*^\wedge$ are exact, which is, surprisingly, not true at higher heights.
	
	\begin{lem}\label{lem: pro-free flat}
	Let $R_* \in \CAlg_*^\wedge$, and let $M_*$ be a pro-free $R_*$-module. Then $M_*$ is flat in $\Mod_{R_*}^\wedge$, that is, the functor $M_* \otimes_{R_*} \cdot$ is exact.
	\end{lem}
	
	\begin{proof}
	If $M_*$ is a pro-free $R_*$-module, it is a coproduct of (possibly shifted) copies of $R_*$ in the category $\Mod^\wedge_{R_*}$. Correspondingly, $M_* \otimes_{R_*} N_*$ is a coproduct of possibly shifted copies of $N_*$, which can be taken in $\Mod^\wedge_*$. The statement follows because coproducts in $\Mod^\wedge_*$ are exact \cite[Proposition 1.9]{HoveySS}.
	\end{proof}
	
	\begin{lem}\label{lem: pro-free base change}
	Pro-freeness is preserved by base change: if $M_*$ is pro-free over $R_*$ and $R_* \to S_*$ is a map of rings in $\Mod_*^\wedge$, then $M_* \otimes_{R_*} S_*$ is pro-free over $S_*$.
	\end{lem}
	
	\begin{proof}
	Again, $M_*$ is a coproduct of copies of $R_*$ in the category $\Mod^\wedge_{R_*}$. The tensor product is a left adjoint, so distributes over this coproduct.
	\end{proof}
	
	\begin{lem}\label{lem: pro-free mod p}
	Suppose that $R_* \in \CAlg_*^\wedge$ and $M_* \in \Mod^\wedge_{R_*}$. Suppose also that $R_*$ is $p$-torsion-free. Then $M_*$ is pro-free over $R_*$ iff $M_*$ is $p$-torsion-free and $M_*/p$ is free over $R_*/p$.
	\end{lem}
	
	\begin{proof}
	Suppose that $M_*$ is pro-free over $R_*$, and write $M_* = L_0\left(\bigoplus_\alpha \Sigma^{n_\alpha} R_*\right)$. By \eqref{eq: L-completion Milnor sequence}, $M_*$ is the same as the $p$-completion of $\bigoplus_\alpha \Sigma^{n_\alpha} R_*$, and is, in particular, $p$-torsion-free. By \cite[Proposition A.4]{HoveyStrickland},
	\[	L_0\left(\bigoplus_\alpha \Sigma^{n_\alpha} R_*\right)/p = \left(\bigoplus_\alpha \Sigma^{n_\alpha} R_*\right)/p = \bigoplus_\alpha \Sigma^{n_\alpha} (R_*/p),	\]
	which is clearly free over $R_*/p$ (and flat, in particular).
	
	For the converse, suppose that $M_*$ is $L$-complete and $p$-torsion-free and $M_*/p$ is free over $R_*/p$. Again using \eqref{eq: L-completion Milnor sequence}, we see that the natural surjection $M_* \to (M_*)^\wedge_p$ is an isomorphism, so that $M_*$ is honestly $p$-complete. Choose generators for $M_*/p$ as an $R_*/p$-module, and lift them to a map
	\[	\phi:F_* \to M_*	\]
	from a free graded $R_*$-module, which is an isomorphism mod $p$. Again, we observe that $L_0(F_*) = (F_*)^\wedge_p$, that it is $p$-torsion-free, and that $L_0(F_*)/p = F_*/p$. Applying the snake lemma to the diagram of graded $\Z_p$-modules
	\[	\xymatrix{ 0 \ar[r] &  L_0(F_*) \ar[d]_{\phi^\wedge} \ar[r]^p & L_0(F_*) \ar[d]^{\phi^\wedge} \ar[r] & F_*/p \ar[d] \ar[r] & 0 \\
				0 \ar[r] & M_* \ar[r]^p & M_* \ar[r] & M_*/p \ar[r] & 0, }	\]
	we see that multiplication by $p$ is an isomorphism on $\ker(\phi^\wedge)$ and $\coker(\phi^\wedge)$. Both of these are $L$-complete graded $\Z_p$-modules, and this implies that they are zero, by \cite[Theorem A.6(d,e)]{HoveyStrickland}.	
	\end{proof}
	
	\begin{lem}
	Let $R$ be a homotopy commutative $K(1)$-local ring spectrum, and let $M$ be a $K(1)$-local $R$-module. Then $M_*$ is pro-free over $R_*$ if and only if there is an equivalence of $K(1)$-local $R$-modules,
	\[	M \simeq \bigvee \Sigma^{n_\alpha}R.	\]
	\end{lem}
	
	(Here, as always, the coproduct is taken in the $K(1)$-local category).
	
	\begin{proof}
	Suppose that $M_*$ is pro-free over $R_*$. Choose generators $x_\alpha \in M_{n_\alpha}$ such that the natural map
	\[	R_*\{x_\alpha\} \to M_*	\]
	becomes an isomorphism after $L$-completion. Each $x_\alpha$ corresponds to a map of spectra $S^{n_\alpha} \to M$, and they assemble to a map of $K(1)$-local $R$-modules
	\[	\bigvee \Sigma^{n_\alpha} R \to M.	\]
	This is an equivalence by a result of Hovey \cite[Theorem 7.3]{HoveySS}, which states that the functor $\pi_*$ sends ($K(1)$-local) coproducts to ($L$-complete) direct sums. The converse also follows from Hovey's result.
	\end{proof}
	
	\begin{rmk}
	A key step in Hovey's proof is that direct sums are exact in $\Mod^\wedge_{KO_*}$, which is specific to height 1 (that is, it has to do with the fact that we are $L$-completing with respect to a principal ideal). Care should thus be taken when attempting to use these techniques at higher heights.
	\end{rmk}
	
	\begin{prop}\label{prop: pro-free tensor}
	Suppose that $R$ is a $K(1)$-local $E_\infty$-algebra and $M$ and $N$ are $R$-modules, such that $M_*$ is pro-free over $R_*$. Then the natural map of $L$-complete modules,
	\[	M_* \otimes_{R_*} N_* \to \pi_*(M \sma_R N),	\]
	is an isomorphism.
	\end{prop}
	
	\begin{proof}
	By the previous lemma, we can write $M$ as a wedge of suspensions of $R$, 
	\[	M \simeq \bigvee \Sigma^{n_\alpha}R \simeq R \sma \bigvee S^{n_\alpha}	\]
	(using the fact that the $K(1)$-local smash product is a left adjoint, so distributes over the $K(1)$-local coproduct). Thus,
	\[	M \sma_R N \simeq N \sma \bigvee S^{n_\alpha} \simeq \bigvee \Sigma^{n_\alpha} N.	\]
	Using Hovey's theorem again \cite[Theorem 7.3]{HoveySS}, we obtain
	\[	\pi_*(M \sma_R N) \cong L_0\left(\bigoplus \Sigma^{n_\alpha} N_*\right) \cong L_0(F_* \otimes_{R_*} N_*),	\]
	where $F_*$ is the free graded $R_*$-module on generators in the degrees $n_\alpha$. By \cite[A.7]{HoveyStrickland},
	\[	\pi_*(M \sma_R N) \cong L_0(L_0(F_*) \otimes_{R_*} N_*) \cong M_* \overline{\otimes}_{R_*} N_*.	\]
	It is clear that this isomorphism is induced by the natural map.
	\end{proof}
	
	We now turn to the problem of homological algebra over an $L$-complete Hopf algebroid. We begin with some definitions generalizing those of \cite{Baker}.
	
	\begin{defn}
	A \textbf{$L$-complete Hopf algebroid} is a cogroupoid object $(R_*, \Gamma_*)$ in $\CAlg_*^\wedge$, such that $\Gamma_*$ is pro-free as a left $R_*$-module. As usual, we write 
	\begin{align*}
		\eta_L, \eta_R: R_* &\to \Gamma_*  &\text{ for the left and right units,} \\
		\Delta: \Gamma_* &\to \Gamma_* \otimes_{R_*} \Gamma_* &\text{ for the comultiplication,} \\
		\epsilon: \Gamma_* &\to R_* &\text{ for the counit, and} \\
		\chi: \Gamma_* &\to \Gamma_* &\text{ for the antipode.}
	\end{align*}
	\end{defn}
	
	Note that $\chi$ gives an isomorphism between $\Gamma_*$ as a left $R_*$-module and $\Gamma_*$ as a right $R_*$-module, so that $\Gamma_*$ is also pro-free as a right $R_*$-module.
	
	\begin{rmk}
	At heights higher than 1, one has to deal with the fact that the left and right units generally do not act in the same way on the generators $(p, u_1, \dotsc, u_{n-1})$ with respect to which $L$-completeness is defined. Thus, Baker's definition has the additional condition that the ideal $(p, u_1, \dotsc, u_{n-1})$ is invariant. At height 1, this condition is trivial.
	\end{rmk}
	
	\begin{defn}
	Let $(R_*, \Gamma_*)$ be an $L$-complete Hopf algebroid. A \textbf{left comodule} over $(R_*, \Gamma_*)$ (a \textbf{left $\Gamma_*$-comodule} for short) is $M_* \in \Mod^\wedge_{R_*}$ together with a coaction map
	\[	\psi: M_* \to \Gamma_* \otimes_{R_*} M_*	\]
	such that the diagrams
	\[	\xymatrix{ M_* \ar[r]^-{\psi} \ar[d]_{\psi} & \Gamma_* \otimes_{R_*} M_* \ar[d]^{\psi \otimes 1} & M_* \ar@{=}[dr] \ar[r]^-{\psi} & \Gamma_* \otimes_{R_*} M_* \ar[d]^{\epsilon \otimes 1}  \\
		\Gamma_* \otimes_{R_*} M_* \ar[r]_-{1 \otimes \Delta} & \Gamma_* \otimes_{R_*} \Gamma_* \otimes_{R_*} M_* & & M_*}	\]
	commute. Write $\Comod^\wedge_{\Gamma_*}$ for the category of left $\Gamma_*$-comodules.
	\end{defn}
	
	\begin{lem}
	The category of left $\Gamma_*$-comodules is abelian, and the forgetful functor $\Comod^\wedge_{\Gamma_*} \to \Mod^\wedge_{\Gamma_*}$ preserves exact sequences.
	\end{lem}
	
	\begin{proof}
	Suppose that
	\[	0 \to K_* \to M_* \stackrel{f}{\to} N_* \to 0	\]
	is an exact sequence of $R_*$-modules, and $f$ is a map of $\Gamma_*$-comodules. A coaction map can then be defined on $K_*$ via the diagram
	\[	\xymatrix{ 0 \ar[r] & K_* \ar@{-->}[d] \ar[r] & M_* \ar[d] \ar[r]^f & N_* \ar[d] \ar[r] & 0 \\
		0 \ar[r] & \Gamma_* \otimes_{R_*} K_* \ar[r] & \Gamma_* \otimes_{R_*} M_* \ar[r] & \Gamma_* \otimes_{R_*} N_* \ar[r] & 0. }	\]
	The bottom sequence is exact because $\Gamma_*$ is flat in $\Mod_{R_*}^\wedge$, by \Cref{lem: pro-free flat}. One checks that this structure makes $K_*$ a comodule by the usual diagram chase. A similar proof works for cokernels.
	\end{proof}

